Scalable Framework for Classifying AI-Generated Content Across Modalities

The rapid growth of generative AI technologies has heightened the importance of effectively distinguishing between human and AI-generated content, as well as classifying outputs from diverse generative models. This paper presents a scalable framework that integrates perceptual hashing, similarity measurement, and pseudo-labeling to address these challenges. Our method enables the incorporation of new generative models without retraining, ensuring adaptability and robustness in dynamic scenarios. Comprehensive evaluations on the Defactify4 dataset demonstrate competitive performance in text and image classification tasks, achieving high accuracy across both distinguishing human and AI-generated content and classifying among generative methods. These results highlight the framework's potential for real-world applications as generative AI continues to evolve. Source codes are publicly available at https://github.com/ffyyytt/defactify4.

==> figures/_flow.tex <==
\usetikzlibrary{shapes.geometric}

\begin{tikzpicture}[square/.style={regular polygon,regular polygon sides=4}]

\draw[->] (-3.5,0) -- (3.5,0) node[right] {$x$};
\draw[->] (0,-3.5) -- (0,3.5) node[above] {$y$};

\node at (-0, 5.5) {\LARGE Stored Features};

\foreach \i in {-10,...,15} {
\pgfmathsetmacro{\t}{\i * 1.8};
\pgfmathsetmacro{\x}{3*cos(\t)};
\pgfmathsetmacro{\y}{3*sin(\t)};
\fill[red] (\x, \y) circle (0.03);}

\foreach \i in {25,...,45} {
\pgfmathsetmacro{\t}{\i * 1.8};
\pgfmathsetmacro{\x}{3*cos(\t)};
\pgfmathsetmacro{\y}{3*sin(\t)};
\fill[blue] (\x, \y) circle (0.03);}

\foreach \i in {55,...,70} {
\pgfmathsetmacro{\t}{\i * 1.8};
\pgfmathsetmacro{\x}{3*cos(\t)};
\pgfmathsetmacro{\y}{3*sin(\t)};
\fill[green] (\x, \y) circle (0.03);}

\foreach \i in {85,...,105} {
\pgfmathsetmacro{\t}{\i * 1.8};
\pgfmathsetmacro{\x}{3*cos(\t)};
\pgfmathsetmacro{\y}{3*sin(\t)};
\fill[yellow] (\x, \y) circle (0.03);}

\foreach \i in {135,...,165} {
\pgfmathsetmacro{\t}{\i * 1.8};
\pgfmathsetmacro{\x}{3*cos(\t)};
\pgfmathsetmacro{\y}{3*sin(\t)};
\fill[purple] (\x, \y) circle (0.03);}

\draw[->] (-8,0) -- (-4.5,0) node[midway, above] {\LARGE k-Nearest Neighbor};


\node at (-11, 5.5) {\LARGE Extracted Features};

\node[fill=red] at (-10,4.33) [square,draw] {};
\node[fill=red] at (-10,4) [square,draw] {};
\node[fill=red] at (-10,3.66) [square,draw] {};

\node[fill=red] at (-11,4.33) [square,draw] {};
\node[fill=red] at (-11,4) [square,draw] {};
\node[fill=red] at (-11,3.66) [square,draw] {};

\node[fill=red] at (-12,4.33) [square,draw] {};
\node[fill=red] at (-12,4) [square,draw] {};
\node[fill=red] at (-12,3.66) [square,draw] {};

\draw[red] (-11,4) ellipse (2cm and 0.7cm);

\node[fill=blue] at (-10,2.33) [square,draw] {};
\node[fill=blue] at (-10,2) [square,draw] {};
\node[fill=blue] at (-10,1.66) [square,draw] {};

\node[fill=blue] at (-11,2.33) [square,draw] {};
\node[fill=blue] at (-11,2) [square,draw] {};
\node[fill=blue] at (-11,1.66) [square,draw] {};

\node[fill=blue] at (-12,2.33) [square,draw] {};
\node[fill=blue] at (-12,2) [square,draw] {};
\node[fill=blue] at (-12,1.66) [square,draw] {};

\draw[blue] (-11,2) ellipse (2cm and 0.7cm);

\node[fill=purple] at (-10,0.33) [square,draw] {};
\node[fill=purple] at (-10,-0) [square,draw] {};
\node[fill=purple] at (-10,-0.33) [square,draw] {};

\node[fill=purple] at (-11,0.33) [square,draw] {};
\node[fill=purple] at (-11,-0) [square,draw] {};
\node[fill=purple] at (-11,-0.33) [square,draw] {};

\node[fill=purple] at (-12,0.33) [square,draw] {};
\node[fill=purple] at (-12,-0) [square,draw] {};
\node[fill=purple] at (-12,-0.33) [square,draw] {};

\draw[purple] (-11,-0) ellipse (2cm and 0.7cm);

\node[fill=green] at (-10,-2.33) [square,draw] {};
\node[fill=green] at (-10,-2) [square,draw] {};
\node[fill=green] at (-10,-1.66) [square,draw] {};

\node[fill=green] at (-11,-2.33) [square,draw] {};
\node[fill=green] at (-11,-2) [square,draw] {};
\node[fill=green] at (-11,-1.66) [square,draw] {};

\node[fill=green] at (-12,-2.33) [square,draw] {};
\node[fill=green] at (-12,-2) [square,draw] {};
\node[fill=green] at (-12,-1.66) [square,draw] {};

\draw[green] (-11,-2) ellipse (2cm and 0.7cm);

\node[fill=yellow] at (-10,-4.33) [square,draw] {};
\node[fill=yellow] at (-10,-4) [square,draw] {};
\node[fill=yellow] at (-10,-3.66) [square,draw] {};

\node[fill=yellow] at (-11,-4.33) [square,draw] {};
\node[fill=yellow] at (-11,-4) [square,draw] {};
\node[fill=yellow] at (-11,-3.66) [square,draw] {};

\node[fill=yellow] at (-12,-4.33) [square,draw] {};
\node[fill=yellow] at (-12,-4) [square,draw] {};
\node[fill=yellow] at (-12,-3.66) [square,draw] {};

\draw[yellow] (-11,-4) ellipse (2cm and 0.7cm);

\node[inner sep=0pt] (russell) at (-34,4)
    {\includegraphics[width=0.04\textwidth]{images/midjourney_1.jpg}};
    
\node[inner sep=0pt] (russell) at (-33,4)
    {\includegraphics[width=0.04\textwidth]{images/midjourney_2.jpg}};
    
\node[inner sep=0pt] (russell) at (-32,4)
    {\includegraphics[width=0.04\textwidth]{images/midjourney_3.jpg}};

\draw[red] (-33,4) ellipse (2cm and 0.7cm);
\node[below] at (-37, 4.33) {\LARGE midjourney};

\node[inner sep=0pt] (russell) at (-34,2)
    {\includegraphics[width=0.04\textwidth]{images/dalle_1.jpg}};
    
\node[inner sep=0pt] (russell) at (-33,2)
    {\includegraphics[width=0.04\textwidth]{images/dalle_2.jpg}};
    
\node[inner sep=0pt] (russell) at (-32,2)
    {\includegraphics[width=0.04\textwidth]{images/dalle_3.jpg}};
    
\draw[blue] (-33,2) ellipse (2cm and 0.7cm);
\node[below] at (-37, 2.33) {\LARGE dalle};

\node[inner sep=0pt] (russell) at (-34,0)
    {\includegraphics[width=0.04\textwidth]{images/real_1.jpg}};
    
\node[inner sep=0pt] (russell) at (-33,0)
    {\includegraphics[width=0.04\textwidth]{images/real_2.jpg}};
    
\node[inner sep=0pt] (russell) at (-32,0)
    {\includegraphics[width=0.04\textwidth]{images/real_3.jpg}};
    
\draw[purple] (-33,0) ellipse (2cm and 0.7cm);
\node[below] at (-37, 0.33) {\LARGE real};

\node[inner sep=0pt] (russell) at (-34,-2)
    {\includegraphics[width=0.04\textwidth]{images/sdxl_1.jpg}};
    
\node[inner sep=0pt] (russell) at (-33,-2)
    {\includegraphics[width=0.04\textwidth]{images/sdxl_2.jpg}};
    
\node[inner sep=0pt] (russell) at (-32,-2)
    {\includegraphics[width=0.04\textwidth]{images/sdxl_3.jpg}};
    
\draw[green] (-33,-2) ellipse (2cm and 0.7cm);
\node[below] at (-37, -1.66) {\LARGE sdxl};

\node[inner sep=0pt] (russell) at (-34,-4)
    {\includegraphics[width=0.04\textwidth]{images/sd21_1.jpg}};
    
\node[inner sep=0pt] (russell) at (-33,-4)
    {\includegraphics[width=0.04\textwidth]{images/sd21_2.jpg}};
    
\node[inner sep=0pt] (russell) at (-32,-4)
    {\includegraphics[width=0.04\textwidth]{images/sd21_3.jpg}};
    
\draw[yellow] (-33,-4) ellipse (2cm and 0.7cm);
\node[below] at (-37, -3.66) {\LARGE sd21};

\node at (-34.5, 5.5) {\LARGE Input Training Images};


\draw[->] (-16,0) -- (-14,0) node[midway, above] {};

\draw[] (-16,0) -- (-16,-3.2) node[midway, above] {};
\draw[->] (-16,-3.2) -- (-30,-3.2) node[midway, above] {};
\node at (-27,-3.8) {\LARGE Pseudo-labeling};
\draw[] (-38.8, -4.8, 0) rectangle ++(8.5,10,0) node[midway] {};
    
\draw[->] (-30,0) -- (-28,0) node[midway, above] {};

\draw[fill=cyan] (-26, -2, 0) rectangle ++(0.2,4,0) node[midway] {};
\draw[fill=cyan] (-25, -1.5, 0) rectangle ++(0.2,3,0) node[midway] {};
\draw[fill=cyan] (-24, -1, 0) rectangle ++(0.2,2,0) node[midway] {};
\draw[fill=cyan] (-23, -0.5, 0) rectangle ++(0.2,1,0) node[midway] {};

\draw[] (-27, -2.5, 0) rectangle ++(5.2,5,0) node[midway] {};
\node at (-24.5, 5.5) {\LARGE Backbone Model};


\draw[->] (-21,0) -- (-20,0) node[midway, above] {};

\draw[->] (-18,-1.5) -- (-18,1.5) node[above] {$W_{y_i}$};

\pgfmathsetmacro{\t}{37 * 1.8};
\pgfmathsetmacro{\x}{-18 + 3*cos(\t)};
\pgfmathsetmacro{\y}{-1.5 + 3*sin(\t)};

\draw[orange] (-18,-1.5) -- (\x, \y) node[above] {$x_i$};
\draw[orange] (-18,-1.5) ++(\t:0.5) arc[start angle=0, end angle=89, radius=0.2];
\node at (-17.7, -0.2) {$\theta_{y_i}$};


\pgfmathsetmacro{\t}{63 * 1.8};
\pgfmathsetmacro{\x}{-18 + 3*cos(\t)};
\pgfmathsetmacro{\y}{-1.5 + 3*sin(\t)};

\draw[orange] (-18,-1.5) -- (\x, \y) node[above] {};


\foreach \i in {30,...,70} {
\pgfmathsetmacro{\t}{\i * 1.8};
\pgfmathsetmacro{\x}{-18 + 3*cos(\t)};
\pgfmathsetmacro{\y}{-1.5 + 3*sin(\t)};
\fill[lime] (\x, \y) circle (0.03);}

\pgfmathsetmacro{\t}{70 * 1.8};
\pgfmathsetmacro{\x}{-18 + 3*cos(\t)};
\pgfmathsetmacro{\y}{-1.5 + 3*sin(\t)};

\draw[lime] (-18,-1.5) -- (\x, \y) node[above] {};


\pgfmathsetmacro{\t}{30 * 1.8};
\pgfmathsetmacro{\x}{-18 + 3*cos(\t)};
\pgfmathsetmacro{\y}{-1.5 + 3*sin(\t)};

\draw[lime] (-18,-1.5) -- (\x, \y) node[above] {};
\draw[lime] (-18,-1.5) ++(\t:0.8) arc[start angle=0, end angle=45, radius=0.3];
\node at (-17.2, -0.1) {m};

\node at (-18, 5.5) {\LARGE ArcFace Loss};


\draw[fill=cyan, opacity=0.1] (-39, -4.9, 0) rectangle ++(43,11,0) node[midway] {};
\node[blue] at (-19, -4.5) {\huge Training Phase};




\draw[fill=cyan, opacity=0.1] (-39, -14, 0) rectangle ++(43,8.9,0) node[midway] {};
\node[blue] at (-19, -13.7) {\huge New Label Adaptation};

\node at (-34.5, -5.6) {\LARGE New Label Inputs};

\node[inner sep=0pt] (russell) at (-34,-10)
    {\includegraphics[width=0.04\textwidth]{images/sd3_1.jpg}};
    
\node[inner sep=0pt] (russell) at (-33,-10)
    {\includegraphics[width=0.04\textwidth]{images/sd3_2.jpg}};
    
\node[inner sep=0pt] (russell) at (-32,-10)
    {\includegraphics[width=0.04\textwidth]{images/sd3_3.jpg}};

\draw[pink] (-33,-10) ellipse (2cm and 0.7cm);
\node[below] at (-37, -9.66) {\LARGE sd3};

\draw[->] (-30,-10) -- (-28,-10) node[midway, above] {};

\draw[fill=cyan] (-26, -12, 0) rectangle ++(0.2,4,0) node[midway] {};
\draw[fill=cyan] (-25, -11.5, 0) rectangle ++(0.2,3,0) node[midway] {};
\draw[fill=cyan] (-24, -11, 0) rectangle ++(0.2,2,0) node[midway] {};
\draw[fill=cyan] (-23, -10.5, 0) rectangle ++(0.2,1,0) node[midway] {};

\draw[] (-27, -12.5, 0) rectangle ++(5.2,5,0) node[midway] {};
\node at (-24.5, -5.6) {\LARGE Trained Model};

\draw[->] (-21,-10) -- (-14,-10) node[midway, above] {};

\node[fill=pink] at (-10,-10.33) [square,draw] {};
\node[fill=pink] at (-10,-10) [square,draw] {};
\node[fill=pink] at (-10,-9.66) [square,draw] {};

\node[fill=pink] at (-11,-10.33) [square,draw] {};
\node[fill=pink] at (-11,-10) [square,draw] {};
\node[fill=pink] at (-11,-9.66) [square,draw] {};

\node[fill=pink] at (-12,-10.33) [square,draw] {};
\node[fill=pink] at (-12,-10) [square,draw] {};
\node[fill=pink] at (-12,-9.66) [square,draw] {};

\draw[pink] (-11,-10) ellipse (2cm and 0.7cm);

\node at (-11, -5.6) {\LARGE New Label's Features};

\draw[->] (-8,-10) -- (-4.5,-10) node[midway, below] {\LARGE k-Nearest Neighbor};
\draw[] (-0.8,-3.7) -- (-6,-10) node[midway, above] {};

\draw[->] (-3.5,-10) -- (3.5,-10) node[right] {$x$};
\draw[->] (0,-13.5) -- (0,-6.5) node[above] {$y$};

\foreach \i in {-10,...,15} {
\pgfmathsetmacro{\t}{\i * 1.8};
\pgfmathsetmacro{\x}{3*cos(\t)};
\pgfmathsetmacro{\y}{3*sin(\t)-10};
\fill[red] (\x, \y) circle (0.03);}

\foreach \i in {25,...,45} {
\pgfmathsetmacro{\t}{\i * 1.8};
\pgfmathsetmacro{\x}{3*cos(\t)};
\pgfmathsetmacro{\y}{3*sin(\t)-10};
\fill[blue] (\x, \y) circle (0.03);}

\foreach \i in {55,...,70} {
\pgfmathsetmacro{\t}{\i * 1.8};
\pgfmathsetmacro{\x}{3*cos(\t)};
\pgfmathsetmacro{\y}{3*sin(\t)-10};
\fill[green] (\x, \y) circle (0.03);}

\foreach \i in {85,...,105} {
\pgfmathsetmacro{\t}{\i * 1.8};
\pgfmathsetmacro{\x}{3*cos(\t)};
\pgfmathsetmacro{\y}{3*sin(\t)-10};
\fill[yellow] (\x, \y) circle (0.03);}

\foreach \i in {135,...,165} {
\pgfmathsetmacro{\t}{\i * 1.8};
\pgfmathsetmacro{\x}{3*cos(\t)};
\pgfmathsetmacro{\y}{3*sin(\t)-10};
\fill[purple] (\x, \y) circle (0.03);}

\foreach \i in {120,...,115} {
\pgfmathsetmacro{\t}{\i * 1.8};
\pgfmathsetmacro{\x}{3*cos(\t)};
\pgfmathsetmacro{\y}{3*sin(\t)-10};
\fill[pink] (\x, \y) circle (0.03);}

\node at (-0, -5.6) {\LARGE Stored Features};

\draw[black, dashed] (-2.5,-11.55) ellipse (0.3cm and 0.5cm);


\draw[fill=cyan, opacity=0.1] (-39, -22.2, 0) rectangle ++(43,8,0) node[midway] {};
\node[blue] at (-19, -21.4) {\huge Inference Phase};

\node at (-34.5, -14.8) {\LARGE Input Testing Images};

\node[inner sep=0pt] (russell) at (-34,-17)
    {\includegraphics[width=0.04\textwidth]{images/test_1_1.jpg}};
    
\node[inner sep=0pt] (russell) at (-33,-17)
    {\includegraphics[width=0.04\textwidth]{images/test_1_2.jpg}};
    
\node[inner sep=0pt] (russell) at (-32,-17)
    {\includegraphics[width=0.04\textwidth]{images/test_1_3.jpg}};
    
    
\node[inner sep=0pt] (russell) at (-34,-19)
    {\includegraphics[width=0.04\textwidth]{images/test_2_1.jpg}};
    
\node[inner sep=0pt] (russell) at (-33,-19)
    {\includegraphics[width=0.04\textwidth]{images/test_2_2.jpg}};
    
\node[inner sep=0pt] (russell) at (-32,-19)
    {\includegraphics[width=0.04\textwidth]{images/test_2_3.jpg}};
    
\draw[gray] (-33,-18) ellipse (2cm and 2.5cm);

\node[below] at (-37, -17.66) {\LARGE Test};

\draw[->] (-30,-18) -- (-28,-18) node[midway, above] {};

\draw[fill=cyan] (-26, -20, 0) rectangle ++(0.2,4,0) node[midway] {};
\draw[fill=cyan] (-25, -19.5, 0) rectangle ++(0.2,3,0) node[midway] {};
\draw[fill=cyan] (-24, -19, 0) rectangle ++(0.2,2,0) node[midway] {};
\draw[fill=cyan] (-23, -18.5, 0) rectangle ++(0.2,1,0) node[midway] {};

\draw[] (-27, -20.5, 0) rectangle ++(5.2,5,0) node[midway] {};
\node at (-24.5, -14.8) {\LARGE Trained Model};

\draw[->] (-21,-18) -- (-14,-18) node[midway, above] {};

\node[fill=gray] at (-10,-18.33) [square,draw] {};
\node[fill=gray] at (-10,-18) [square,draw] {};
\node[fill=gray] at (-10,-17.66) [square,draw] {};

\node[fill=gray] at (-11,-18.33) [square,draw] {};
\node[fill=gray] at (-11,-18) [square,draw] {};
\node[fill=gray] at (-11,-17.66) [square,draw] {};

\node[fill=gray] at (-12,-18.33) [square,draw] {};
\node[fill=gray] at (-12,-18) [square,draw] {};
\node[fill=gray] at (-12,-17.66) [square,draw] {};

\node at (-11, -14.8) {\LARGE Testing's Features};

\draw[->] (-8,-18) -- (-4.5,-18) node[midway, below] {\LARGE k-Nearest Neighbor};
\draw[] (-0.8,-13.7) -- (-6,-18) node[midway, above] {};

\draw[] (-2.5, -19, 0) rectangle ++(5,2,0) node[midway] {};
\node at (0, -18) {\LARGE Output predictions};

\end{tikzpicture}
